Thresholded Lasso Bandit

In this paper, we revisit the regret minimization problem in sparse stochastic contextual linear bandits, where feature vectors may be of large dimension $d$, but where the reward function depends on a few, say $s_0\ll d$, of these features only. We present Thresholded Lasso bandit, an algorithm that (i) estimates the vector defining the reward function as well as its sparse support, i.e., significant feature elements, using the Lasso framework with thresholding, and (ii) selects an arm greedily according to this estimate projected on its support. The algorithm does not require prior knowledge of the sparsity index $s_0$ and can be parameter-free under some symmetric assumptions. For this simple algorithm, we establish non-asymptotic regret upper bounds scaling as $\mathcal{O}( \log d + \sqrt{T} )$ in general, and as $\mathcal{O}( \log d + \log T)$ under the so-called margin condition (a probabilistic condition on the separation of the arm rewards). The regret of previous algorithms scales as $\mathcal{O}( \log d + \sqrt{T \log (d T)})$ and $\mathcal{O}( \log T \log d)$ in the two settings, respectively. Through numerical experiments, we confirm that our algorithm outperforms existing methods.

==> Lasso Bandits_arXiv/abstract.tex <==

\begin{abstract}
 In this paper, we revisit the regret minimization problem in sparse stochastic contextual linear bandits, where feature vectors may be of large dimension $d$, but where the reward function depends on a few, say $s_0\ll d$, of these features only. We present Thresholded Lasso bandit, an algorithm that (i) estimates the vector defining the reward function as well as its sparse support, i.e., significant feature elements, using the Lasso framework with thresholding, and (ii) selects an arm greedily according to this estimate projected on its support. The algorithm does not require prior knowledge of the sparsity index $s_0$ and can be parameter-free under some symmetric assumptions. For this simple algorithm, we establish non-asymptotic regret upper bounds scaling as $\mathcal{O}( \log d + \sqrt{T} )$ in general, and as $\mathcal{O}( \log d + \log T)$ under the so-called margin condition (a probabilistic condition on the separation of the arm rewards). The regret of previous algorithms scales as $\mathcal{O}( \log d + \sqrt{T \log (d T)})$ and $\mathcal{O}( \log T \log d)$ in the two settings, respectively. Through numerical experiments, we confirm that our algorithm outperforms existing methods. 
\end{abstract}


==> Lasso Bandits_arXiv/contents.tex <==

\section{Introduction}

The linear contextual bandit \cite{abe1999, li2010contextual} is a sequential decision-making problem that generalizes the classical stochastic Multi-Armed Bandit (MAB) problem \cite{lai1985asymptotically,robbins1952some}, where (i) in each round, the decision-maker is provided with a {\it context} in the form of a feature vector for each arm and where (ii) the expected reward is a linear function of these vectors. More precisely, at the beginning of round $t\ge 1$, the decision-maker receives for each arm $k$, a feature vector $A_{t, k}\in \mathbb{R}^d$. She then selects an arm, say $k$, and observes a sample of a random reward with mean $\langle A_{t,k}, \theta\rangle$. The parameter vector $\theta\in \mathbb{R}^d$ is fixed but initially unknown. Linear contextual bandits have been extensively applied in online services such as online advertisement and recommendation systems \cite{li2010contextual, li2016collaborative, zeng2016online}, and constitute arguably the most relevant structured bandit model in practice.

The major challenge in the design of efficient algorithms for contextual linear bandits stems from the high dimensionality of the feature space. For example, for display ad systems as studied in \citet{chapelle2011empirical,weinberger2009}, the joint information about a user, an ad and its publisher is encoded in a feature vector of dimension $d=2^{24}$. Fortunately, typically only a few features significantly impact the expected reward. This observation has motivated the analysis of problems where the unknown parameter vector $\theta$ is sparse \cite{Bastani2015,kim2019doubly, oh2020sparsity,wang2018minimax}. In this paper, we also investigate  sparse contextual linear bandits, and assume that $\theta$ only has at most $s_0\ll d$ non-zero components. The set of these components and its cardinality $s_0$ are unknown to the decision-maker. Sparse contextual linear bandits have attracted a lot of attention recently. State-of-the-art algorithms developed to exploit the sparse structure achieve regrets scaling as $\mathcal{O}( \log d + \sqrt{T \log (dT)})$ in general, and $ \mathcal{O}( \log d \log T)$ under the co-called margin condition (a setting where arms are well separated); refer to Section \ref{sec:related} for details.              

We develop a novel algorithm, referred to as Thresholded Lasso bandit\footnote{An implementation of our method is available at \url{https://github.com/CyberAgentAILab/thresholded-lasso-bandit}.}, with improved regret guarantees. Our algorithm first uses the Lasso framework with thresholding to maintain and update in each round estimates of the parameter vector $\theta$ and of its support. It then greedily picks an arm based on these estimates (the {\it thresholded} estimates of $\theta$). The regret of the algorithm strongly depends on the accuracy of these estimates. We derive strong guarantees on this accuracy, which in turn leads to regret guarantees. Our contributions are as follows.

\paragraph{(i) Thresholded Lasso Estimation Performance.} The performance of the Lasso-based estimation procedure is now fairly well understood, see e.g., \citet{buhlmann2011statistics,tibshirani1996regression, zhou2010thresholded}. For example, \citet{zhou2010thresholded} provides an analysis of the estimation of the support of $\theta$, and specifically, gives upper bounds on the number of false positives (components that are not in the support, but estimated as part of it) and false negatives (components that are in the support, but not estimated as part of it). These analyses, however, critically rely on the assumption that the observed data is i.i.d.. This assumption does not hold for the bandit problem, as the algorithm adapts its arm selection strategy depending on the past observations. Despite the non i.i.d. nature of the data, we manage to derive performance guarantees of the estimate of $\theta$. In particular, we establish high probability guarantees that are independent of the dimension $d$ (see Lemma~\ref{lm:LS_estim_risk_klarge}).

\paragraph{(ii) Regret Guarantees.} Based on the analysis of the Thresholded Lasso estimation procedure, we provide a finite-time analysis of the regret of our algorithm under certain symmetry assumptions made in \citet{oh2020sparsity}. 
The regret scales at most as ${\mathcal{O}}( \log d + \sqrt{T} )$ in general and ${\mathcal{O}}(\log d + \log T)$ under the margin condition. More precisely, the estimation error of $\theta$ induces a regret scaling as $\mathcal{O}( \sqrt{ T})$ (or $ \mathcal{O}( \log T)$ under the margin condition). The additional term $ \mathcal{O}(\log d )$ in our regret upper bounds comes from the errors made when estimating the support of $\theta$. It is worth noting that when using the plain Lasso estimator (without thresholding), one would obtain weaker performance guarantees for the estimation of $\theta$, typically depending on $d$, see e.g., \citet{Bastani2015}. This dependence causes an additional multiplicative term $\log d$ in the regret.

\paragraph{(iii) Numerical Experiments.} We present extensive numerical experiments to illustrate the performance of the Thresholded Lasso bandit algorithm. We compare the estimation accuracy for $\theta$ and the regret of our algorithm to those of the Lasso bandit, Doubly-Robust Lasso bandit, and Sparsity-Agnostic Lasso bandit algorithms \cite{bastani2020online, kim2019doubly, oh2020sparsity}. These experiments confirm the benefit of the use of the Lasso procedure with thresholding. 



\begin{table*}[t]
\caption{Algorithms and their regret guarantees for scaling with respect to $d$ and $T$. $\mathcal{O}$ notations are hiding sub-logarithmic factors in $d$ and logarithmic factors in $s_0$. The 'Compatibility' and 'Margin' conditions refer to Assumptions \ref{asm:comp_cond} and \ref{asm:margin}.}
\label{tab:related_work}
\vskip 0.15in 
\begin{center}
\begin{tabular}{lcccc}
\toprule
Paper & Regret & 
Compatibility & Margin & Other \\
\midrule
{\small \citet{abbasi2012online}} & ${\mathcal{O}}(d s_0 (\log { T})^2)$ & & & \\
{\small \citet{bastani2020online}}  & $\mathcal{O}(s_0^2(\log d + \log T)^2)$ & \boldcheckmark  & \boldcheckmark &   \\
{\small \citet{wang2018minimax}}   & $\mathcal{O}(s_0^2( \log d + s_0) \log T)$ & \boldcheckmark  & \boldcheckmark  & \\
{\small \citet{kim2019doubly}} & $\mathcal{O}(s_0 \sqrt{T} \log (d T))$ & \boldcheckmark   &  & \\
{\small \citet{ren2020dynamic}} & {\small $\mathcal{O}(s_0 \mbox{polylog}(d) + \log(T)\sqrt{s_0T \log d })$} &    &  & {\small Restricted Bounded Density}
\\
{\small  \citet{oh2020sparsity}}   & $\mathcal{O} ( s_0^2 \log d + s_0 \sqrt{T \log (dT)})$& \boldcheckmark  &  & Asm \ref{asm:relax_sym}, \ref{asm:balanced_cov} \\
{\small This work: Theorem~\ref{thm:regret_ub_klarge}}&  $\mathcal{O}(s_0^2\log d  +  s_0\log T)$ & \boldcheckmark & \boldcheckmark & Asm \ref{asm:relax_sym}, \ref{asm:balanced_cov}, \ref{asm:cov_div_klarge}\\
{\small This work: Theorem~\ref{thm:regret_ub_wo_margin_klarge}}& $\mathcal{O}(s_0^2 \log d  +  
\sqrt{s_0 T })$& \boldcheckmark  &  & 
Asm \ref{asm:relax_sym}, \ref{asm:balanced_cov}, \ref{asm:cov_div_klarge} 
\\
\begin{tabular}{c}
{\small \citet{bastani2021mostly}}\\
{\small (non-sparse setting) }
\end{tabular}
& $\mathcal{O}(d \log d \log T)$ & & \boldcheckmark  & 
\begin{tabular}{c}
{\small Covariate diversity condition}\\
{\small (Stronger than Asm~\ref{asm:cov_div_klarge})}
\end{tabular}
\\
\bottomrule
\end{tabular}
\end{center}
\vskip -0.1in
\end{table*}

\section{Related Work}\label{sec:related}
 
Stochastic linear bandit problems have attracted a lot of attention over the last decade. \citet{carpentier2012bandit} addresses sparse linear bandits where  $\|\theta\|_0 \le s_0$ and where the set of arms is restricted to the $\ell_2$ unit ball. For regimes where the time horizon is much smaller than the dimension $d$, i.e., $T \ll d$, the authors propose an algorithm whose regret scales at most as ${\mathcal{O}}(s_0\sqrt{T} \log(d T))$. \citet{botao2020high} studied high-dimensional linear bandit problems where the number of actions is larger than or equal to $d$. Under some signal strength conditions, they propose an algorithm that achieves a regret of $\mathcal{O}(s_0 \log d + \sqrt{s_0 T \log (dT)})$. These studies, however, do not consider problems with contextual information.
    
Recently, high-dimensional contextual linear bandits have been investigated under the sparsity assumption $\|\theta\|_0 \le s_0$. In this line of research, the decision-maker is provided in each round with a set of arms defined by a finite set of feature vectors. This set is uniformly bounded across rounds. In this setting, the authors of \citet{abbasi2012online} devise an algorithm with both a minimax (problem independent) regret upper bound $\tilde{\mathcal{O}}(\sqrt{s_0 dT})$ and problem dependent upper bound ${\mathcal{O}}(d s_0 (\log { T})^2)$ (the notation $\tilde{\mathcal{O}}$ hides the polylogarithmic terms) without any assumption on the distribution (other than the assumptions similar to our Assumption~\ref{asm:sparsity_param_klarge}).

In \citet{bastani2020online} (initially published in 2015 as \citet{Bastani2015}), the authors address a high-dimensional contextual linear bandit problem where the unknown parameter defining the reward function is arm-specific ($\theta$ is different for the various arms). In the proposed algorithm, arms are explored uniformly at random for $\mathcal{O}( s_0^2 \log d \log T)$ prespecified rounds. Under the margin condition, similar to our Assumption~\ref{asm:margin}, the algorithm achieves a regret of $\mathcal{O}(s_0^2(\log d + \log T)^2)$. For the same problem, \citet{wang2018minimax} develops the so-called MCP-Bandit algorithm. The latter also uses the uniform exploration for $\mathcal{O}( s_0^2 \log d \log T)$ prespecified rounds, and has improved regret guarantees: the regret scales as $\mathcal{O}(s_0^2( \log d + s_0) \log T)$. 
  
High-dimensional contextual linear bandits have been also studied without the margin condition, but with a unique parameter $\theta$ defining the reward function. \citet{kim2019doubly} designs an algorithm with uniform exploration phases of $\mathcal{O}(\sqrt{T  \log(d T) \log T})$ rounds, and with regret $\mathcal{O}(s_0 \sqrt{T} \log (d T))$. All the aforementioned algorithms require the knowledge of the sparsity index $s_0$. In \citet{oh2020sparsity}, the authors propose an algorithm, referred to as SA Lasso bandit, that does not require this knowledge, and with regret $\mathcal{O} (s_0^2 \log d +  s_0 \sqrt{T \log (dT)})$. 
In addition, SA Lasso bandit does not include any uniform exploration phase. Its regret guarantees are derived under specific assumptions on the context distribution, the so-called relaxed symmetry assumption and the balanced covariance assumption. 
The authors also establish a $\mathcal{O}(s_0^2 \log d + \sqrt{s_0 T \log (d T)})$ regret upper bound under the so-called {\it restricted eigenvalue} condition. In \citet{ren2020dynamic}, under the restricted eigenvalue condition induced by the restricted bounded density assumption, the authors established a regret bound of $\mathcal{O}(s_0 \mbox{polylog}(d) + \sqrt{s_0T \log(d) \mbox{polylog}(T)})$.

One notable recent development in contextual bandit is the regret analyses of the exploration-free or greedy algorithms. Under some symmetry assumptions on the context distribution, these algorithms exhibit sub-linear regret  \cite{bastani2021mostly, kannan2018smoothed, ren2020dynamic, oh2020sparsity}.  Our analysis is also inspired by the results on exploration-free algorithms.


In this paper, we develop an algorithm with improved regret guarantees with and without the margin condition. The algorithm does not rely on the knowledge of $s_0$ and can be made parameter-free.  Such a parameter-free algorithm is not proposed in other recent papers. We have summarized the relevant studies and our work in Table~\ref{tab:related_work}. We will come back to this table when we discuss the assumptions.




\section{Model and Assumptions}\label{sec:model}

\subsection{Model and Notation}
 We consider a contextual linear stochastic bandit problem in a high-dimensional space. In each round $t \in [T]:=\{1,\ldots,T\}$, the algorithm is given a set of context vectors $ \mathcal{A}_t = \{ A_{t, k} \in \mathbb{R}^{d}: k \in [K]\}$. The successive sets $( \mathcal{A}_t )_{t \ge 1}$ form an i.i.d. sequence with distribution $p_{{A}}$. In round $t$, the algorithm selects an arm $A_t \in \mathcal{A}_t $ based on past observations, and collects a random reward $r_t$. Formally, if $\mathcal{F}_{t}$ is the $\sigma$-algebra generated by random variables $(\mathcal{A}_1,A_1,r_1, \ldots,\mathcal{A}_{t-1},A_{t-1},r_{t-1}, \mathcal{A}_{t})$, $A_t$ is $\mathcal{F}_{t}$-measurable. We assume that $r_t = \langle A_{t}, \theta\rangle + \varepsilon_t$, where $\varepsilon_t$ is a  zero mean sub-Gaussian random variable with variance proxy $\sigma^2$ given $\mathcal{F}_{t}$ and $A_t$.
Our objective is to devise an algorithm with minimal regret, where regret is defined as: 
 \begin{align*}
 	R(T) & \coloneqq \EXP \left[ \sum_{t =1}^T \max_{A \in \mathcal{A}_t} \langle A, \theta\rangle - r_t\right]
 	\\
 	& =  \EXP \left[ \sum_{t =1}^T \max_{A \in \mathcal{A}_t} \langle A - A_t, \theta\rangle\right].
 \end{align*}

\paragraph{Notation.} The $\ell_0$-norm of a vector $\theta\in \mathbb{R}^d$ is $\|\theta\|_0= \sum_{i = 1}^d  \indicator \left\{ \theta_i \neq 0\right\}$. We denote $\hat{\Sigma}_t = \frac{1}{t}\sum_{s=1}^t A_s A_s^\top$ as the empirical Gram matrix generated by the arms selected under a specific algorithm. For any $B \subset [d]$, we define $\theta_{B} \coloneqq (\theta_{1, B}, \ldots, \theta_{d, B})^\top $ where for all $i \in [d]$, $\theta_{i, B} \coloneqq \theta_i \indicator \{ i \in B\}$.
For each $ B \subset [d]$, we define the submatrix $A(B) \in \mathbb{R}^{n \times |B|}$ of $ A \in \mathbb{R}^{n \times d}$ where for $A(B)$, we extract the rows that are in $B$. We denote $\textnormal{supp}(x)$ as the set of the non-zero element indices of $x\in\mathbb{R}^d$. We also define $\theta_{\min}$ as the minimal value of $|\theta_i|$ on the support: $\theta_{\min} \coloneqq \min_{i \in \text{supp}(\theta)} |\theta_i|$. We denote by $S(\theta)= \text{supp}(\theta) = \{i \in [d] : \theta_i \neq 0\}$ the support of $\theta$. Definitions and notations are also summarized in Appendix~\ref{app:table_of_notations}, Table~\ref{tab:notions}.

\subsection{Assumptions} 

We present a set of assumptions used throughout the paper. 
Many assumptions are essentially from \citet{oh2020sparsity}. However, there are some differences, and these will be discussed.
We also discuss and compare these assumptions to those made in the related literature.  

\begin{assumption}[Sparsity and parameter constraints]\label{asm:sparsity_param_klarge}
The parameter $\theta$ defining the reward function is sparse, i.e., $\| \theta\|_0\le s_0$ for some fixed but unknown integer $s_0$ ($s_0$ does not depend on $d$). 
We further assume that $\|\theta\|_1 \le s_1 $ for some unknown constant\footnote{Given this assumption of $s_1$ to be a constant, note that the value of $\theta_{\min}$ would scale as $\Theta\left(1/s_0\right)$, as $s_0 \theta_{\min} \le \|\theta\|_1 \le s_1 $ may hold. Note that in  \citet{oh2020sparsity}, $\|\theta\|_2 \le \Theta(1)$ and $\|A\|_2 \le \Theta(1)$ (for all $A \in \mathcal{A}_t$) are assumed.} $s_1$  and $\theta_{\min} \ge s_2 /s_0 $ with some unknown constant $s_2\; (< s_1)$.
Finally, we assume that the $\ell_\infty$-norm of the context vector is bounded: for all $t$ and for all $A \in \mathcal{A}_t$, $\|A\|_\infty \le s_A$, where $s_A>0$ is a constant. 
\end{assumption}

\begin{assumption}[Compatibility condition]\label{asm:comp_cond}
  For a matrix $M \in \mathbb{R}^{d \times d}$ and a set $S_0 \subset [d]$, we define the compatibility constant $\phi(M, S_0)$ as:
$$
     \phi^2(M, S_0) \!\coloneqq \!\min_{x:  \|x_{S_0}\|_1 \neq 0} \left\{\! \frac{s_0 x^\top M x}{\|x_{S_0}\|_1^2} \!:\! \|x_{S_0^c}\|_1 \!\le\! 3 \|x_{S_0}\|_1 \!\right\}\!.
$$
We assume that for the Gram matrix of the action set $\Sigma \coloneqq \frac{1}{K} \sum_{k=1}^K \EXP_{\mathcal{A}\sim p_A} \left[A_{k} A_{k}^\top\right]$ satisfies $\phi^2(\Sigma, S(\theta)) \ge \phi^2_0$, where $\phi_0>0$ is some positive constant. 
 \end{assumption}
 The compatibility condition was introduced in the high-dimensional statistics literature \cite{buhlmann2011statistics}. It ensures that the Lasso estimate \cite{tibshirani1996regression} of the parameter $\theta$ approaches to its true value as the number of samples grows large. Note that it is easy to check that the compatibility condition is strictly weaker than assuming the positive definiteness of $\Sigma$. It allows us to consider feature vectors with strongly correlated components.  Assumption~\ref{asm:comp_cond} is considered to be essential for the Lasso estimate to be consistent and assumed in many of the relevant studies. See Table~\ref{tab:related_work} for studies using the compatibility condition. $\phi_0$ can be a constant that does not depend on $d$. This is the case, for example, when the context distribution is multivariate Gaussian, uniform distribution. 
 In these examples, the minimum eigenvalue of the Gram matrix is lower bounded by some constant. When the minimum eigenvalue is lower bounded by some constant, the compatibility constant is also lower bounded by some constant \cite{buhlmann2011statistics}.
 
 \begin{assumption}[Relaxed symmetry \cite{oh2020sparsity}]\label{asm:relax_sym}
 For the distribution $p_A$ of $\mathcal{A}$, there exists a constant $\nu\ge1$ such that for all $\vec{A} \in \mathbb{R}^{K \times d}$ such that $p_A(\vec{A})>0$, $\frac{p_A(\vec{A})}{p_A(- \vec{A})} \le \nu$.
 \end{assumption}
 
\begin{assumption}[Balanced covariance \cite{oh2020sparsity}]\label{asm:balanced_cov}
For any permutation $\gamma$ of $[K]$,  for any integer $k \in \{2,...,K-1\}$ and a fixed $\theta$, there exists a constant $C_{\textnormal{b}}> 1$ such that
\small
\begin{align*}
    & C_{\textnormal{b}}  \mathbb{E}_{\mathcal{A} \sim p_A} \left[ ( A_{\gamma(1)} A^\top_{\gamma(1)} + A_{\gamma(K)} A^\top_{\gamma(K)}) \right.
    \\
    & \qquad \qquad \quad \left. \cdot \indicator \{ \langle A_{\gamma(1)},  \theta \rangle < \ldots < \langle A_{\gamma(K)}, \theta \rangle \} \right]
    \\
    &\succeq \mathbb{E}_{\mathcal{A} \sim p_A}\left[ A_{\gamma(k)} A^\top_{\gamma(k)}  \indicator \{ \langle A_{\gamma(1)}, \theta \rangle < \ldots < \langle A_{\gamma(K)}, \theta \rangle \} \right].
\end{align*}
\normalsize
\end{assumption}

\begin{assumption}[Sparse positive definiteness]\label{asm:cov_div_klarge}
Define for each $B \subset [d]$,
$
\Sigma_B \coloneqq \frac{1}{K} \sum_{k=1}^K \EXP_{\mathcal{A}\sim p_A} \left[A_{k}(B) A_{k}(B)^\top\right],
$
where $ A_{k}(B)$ is a $|B|$-dimensional vector, which is extracted from the elements of $A_{k}$ with indices in $B$.  There exists a positive constant $\alpha>0$ such that $\forall B \subset [d]$,
 \begin{align*}
 & |B| \le s_0 + (4 \nu C_{\textnormal{b}}\sqrt{s_0})/\phi_0^2 \; \text{and} \; S(\theta) \subset B 
 \\
 & \qquad \Longrightarrow  \min_{v \in \mathbb{R}^{|B|} : \|v\|_2 = 1} v^\top \Sigma_B v  \ge \alpha.
 \end{align*}
 The parameters $\phi_0, \nu, C_{\textnormal{b}}$ are those of Assumptions \ref{asm:comp_cond}, \ref{asm:relax_sym}, and~\ref{asm:balanced_cov}.
 \end{assumption}
 Assumption~\ref{asm:relax_sym} comes from \citet{oh2020sparsity}. This assumption is satisfied for the wide range of distributions including multivariate Gaussian, uniform, and  Bernoulli distributions. 
 Assumption~\ref{asm:balanced_cov} is also adopted from \citet{oh2020sparsity}. 
 This assumption holds for a wide range of distributions including multivariate Gaussian distribution, uniform distribution on sphere.
It also holds when contexts are independent across arms with any arbitrary distributions \cite{oh2020sparsity}.  Assumption~\ref{asm:cov_div_klarge} implies that the context distribution is diverse enough in the neighborhood of the support of $\theta$. Note that Assumption~\ref{asm:cov_div_klarge} is standard in low dimensional linear bandit literature (e.g., \citet{lattimore2020bandit, degenne2020gamification, jedra2020optimal,hao2020adaptive}). There, if $S(\theta)=[d]$, the only choice for $B$ is $[d]$, and the set of action has to span $\mathbb{R}^d$ (hence Assumption~\ref{asm:cov_div_klarge} is satisfied). 
We will see that after an accurate estimate of the support $S(\theta)$ (Lemma~\ref{lm:support_recovery_klarge}), Assumption~\ref{asm:cov_div_klarge} is used only to analyze the performance of the least square estimator of low-dimensional (order of $\mathcal{O}(s_0)$) vector. Assumption~\ref{asm:cov_div_klarge} is strictly weaker than the covariate diversity condition of \citet{bastani2021mostly}, where the positive definiteness must be guaranteed for the Gram matrix generated by the greedy algorithm.   We also discuss the details of assumptions in Appendix~\ref{app:assumption_K}.

\section{Algorithm} 

 In this section, we present the Thresholded (TH) Lasso bandit algorithm. The algorithm adapts the idea of Lasso with thresholding proposed in \citet{zhou2010thresholded} to estimate $\theta$ and its support. The main challenge in the analysis of the Lasso with thresholding stems from the fact that here, the data is non i.i.d. (the arm selection is adaptive). 




\begin{algorithm}[htb]
  \caption{TH Lasso Bandit}
  \label{algo:th_lasso_bandit}
  \begin{algorithmic}[1]
    \STATE \textbf{Input:} $\lambda_0 $
    \FOR {$t=1,\cdots,T$}
      \STATE Receive a context set $\mathcal{A}_t: = \{A_{t,k} : k \in [K]\}$
      \STATE Pull arm $A_t=\argmax_{A \in \mathcal{A}_t} \langle A, \hat{\theta}_t \rangle$ (ties are broken uniformly at random) and observe $r_t$
      \STATE $\lambda_t \gets  \lambda_0 \sqrt{\frac{2 \log t \log d}{t}}$
      \STATE $A \gets (A_1, A_2, \ldots, A_t)^\top, \quad R \gets (r_1, r_2, \ldots, r_t)^\top$
      \STATE  $\hat{\theta}_0^{(t)} \gets \argmin_{\theta} \frac{1}{t}\|R - A\theta \|_2^2 + \lambda_t \|\theta\|_1$
      \STATE $\hat{S}_0^{(t)} \gets \{j\in [d] :\; |(\hat{\theta}^{(t)}_0)_j| > 4 \lambda_t\}$ 
      \STATE $\hat{S}_1^{(t)} \gets \{j\in \hat{S}_0^{(t)} : \; | (\hat{\theta}^{(t)}_0)_j| \geq 4 \lambda_t \sqrt{|\hat{S}_0^{(t)}|}\}$
      \STATE $A_S \gets (A_{1, \hat{S}_1^{(t)}}, A_{2, \hat{S}_1^{(t)}}, \ldots, A_{t, \hat{S}_1^{(t)}})^\top$
      \STATE $\hat{\theta}_{t+1} \gets \argmin_{\theta}\|R - A_S \theta\|_2^2$
      \ENDFOR
    \end{algorithmic}
\end{algorithm}

The pseudo-code of our algorithm is presented in Algorithm~\ref{algo:th_lasso_bandit}. In round $t$, the algorithm pulls the arm in a greedy way using the estimated value $\hat{\theta}_t$ of $\theta$. From the past selected arms and rewards, we get via the Lasso a first estimate $\hat{\theta}_0^{(t)}$ of $\theta$. This estimate is then used to estimate the support of $\theta$ using appropriate thresholding. The regularizer $\lambda_t \coloneqq \lambda_0 \sqrt{(2 \log t \log d)/t}$ is set at a much larger value than that in  the previous work (they typically have the order of $ \sqrt{(\log d + \log t)/t}$), as we are only focusing on the support recovery here. Note that we apply a thresholding procedure twice to $\hat{\theta}_0^{(t)}$ to provide the support estimate $\hat{S}_1^{(t)}$. The final estimate $\hat{\theta}_{t+1}$ is obtained as the least squares estimator of $\theta$, when restricted to $\hat{S}_1^{(t)}$. The initial support estimate done by Lasso contains too many false positives. By including thresholding steps in the algorithm, we remove the unnecessary false positives and improve the support estimate. We quantify this improvement in the next section.


\section{Performance Guarantees}\label{sec:upper_bounds}

We analyze the regret of the Thresholded Lasso bandit algorithm both when the margin condition holds and when it does not. 
We show that better guarantees can be obtained with a single-parameter or parameter-free algorithm.

\subsection{With the Margin Condition}

 \begin{assumption}[Margin condition]\label{asm:margin}
 There exists a constant $C_{\textnormal{m}} >0$ such that for all $\kappa>0$, 
 \begin{align*}
     \forall k\neq k', \quad \Pr_{A \sim p_{A}}(0 < |\langle A_{k} - A_{k'}, \theta\rangle| \le \kappa) \le C_{\textnormal{m}} \kappa.
 \end{align*}
 \end{assumption}
The margin condition controls the probability that under $p_A$ two arms yield very similar rewards (and hence are hard to separate) and is 
widely used in the classification literature (see e.g., \citet{tsybakov2004optimal, audibert2007fast}). 
For the (low-dimensional) linear bandit literature, it was first introduced in \citet{goldenshluger2013linear}. 
The margin condition holds for the most usual context distributions (including the uniform distribution and Multivariate Gaussian distributions) and a much weaker assumption than requiring the strict separation between the arms.

The following theorem provides a non-asymptotic regret upper bound of TH Lasso bandit under the margin condition. To simplify the presentation of our regret upper bound, define  $\tau = \left\lfloor\frac{2 \log (2 d^2)}{C_0^2} (\log s_0) (\log \log d) \right\rfloor $, where $C_0 =\min \left\{\frac{1}{2}, \frac{\phi_0^2}{512 s_0 s_A^2 \nu C_{\textnormal{b}}}\right\}$.
Note that $\tau = \mathcal{O}\left(s_0^2 (\log s_0) (\log d) (\log \log d)\right)$.
\begin{theorem}\label{thm:regret_ub_klarge}
Assume that Assumptions \ref{asm:sparsity_param_klarge} -- \ref{asm:cov_div_klarge}, \ref{asm:margin} hold.\\
(i) (TH Lasso Bandit with parameter-dependent input) There are universal positive constants $c_1, c_2, c_3$ depending on $ \sigma, s_A, s_1, s_2, \phi_0, \nu, C_{\textnormal{b}},   K,  \alpha, C_{\textnormal{m}}$, such that if we set $\lambda_0=c_1$, then for all $d \ge c_2$, for all $T \ge 2$:
\begin{align*}
& R(T) \le c_3\left( \tau + s_0 (\log s_0)^{\frac{3}{2}}\log T + s_0^2\right).
\end{align*}
(ii) (TH Lasso Bandit with parameter-free input) There are universal positive constants $c_4, c_5$ depending on $ \sigma, s_A, s_1, s_2, \phi_0, \nu, C_{\textnormal{b}},   K,  \alpha, C_{\textnormal{m}}$, such that if we set $ \lambda_0 = {1}/{(\log \log d)^{\frac{1}{4}}}$ in TH Lasso Bandit, then for all $d \ge c_4$, for all $T \ge 2$,
\begin{align*}
     R(T)\le c_5\left( \tau + s_0 (\log s_0)^{\frac{3}{2}}\log T + s_0^2\right).
\end{align*}
The precise definitions of $c_1$-$c_5$ are given in Appendix~\ref{subsec:proof_regret_ub_klarge}.
\end{theorem}
We provide the proof of Theorem~\ref{thm:regret_ub_klarge} in Appendix~\ref{subsec:proof_regret_ub_klarge}. 





 
\subsection{Without the Margin Condition}

\begin{theorem}\label{thm:regret_ub_wo_margin_klarge}
Assume that Assumptions \ref{asm:sparsity_param_klarge} -- \ref{asm:cov_div_klarge} hold.\\
(i) (TH Lasso Bandit with parameter-dependent input) There are universal positive constants $c_1, c_2, c_3$ depending on $ \sigma, s_A, s_1, s_2, \phi_0, \nu, C_{\textnormal{b}},   K,  \alpha$ such that if we set
$\lambda_0 = c_1 $, then for all $d \ge c_2$. for all $T \ge 2$:
\begin{align*}
& R(T) \le c_3\left(  \tau +  (\log s_0) \sqrt{s_0 T} + s_0^2\right).
\end{align*}
(ii) (TH Lasso Bandit with parameter-free input) There are universal positive constants $c_4, c_5$ depending on $ \sigma, s_A, s_1, s_2, \phi_0, \nu, C_{\textnormal{b}},   K,  \alpha$ such that if we set $ \lambda_0 = {1}/{(\log \log d)^{\frac{1}{4}}}$ in TH Lasso Bandit, then for all $d \ge c_4$, for all $T \ge 2$,
\begin{align*}
     R(T)\le c_5\left( \tau +  (\log s_0) \sqrt{s_0 T} + s_0^2\right).
\end{align*}
The precise definitions of $c_1$-$c_5$ are given in Appendix~\ref{subsec:regret_ub_wo_margin_klarge}
\end{theorem}
The proof of Theorem~\ref{thm:regret_ub_wo_margin_klarge} is presented in Appendix~\ref{subsec:regret_ub_wo_margin_klarge}.



Theorems \ref{thm:regret_ub_klarge} and \ref{thm:regret_ub_wo_margin_klarge} state that TH Lasso bandit achieves much lower regret than the existing algorithms. Indeed, upper regret bounds for the latter had a term scaling as $\log d \log T$ (resp. $\log d + \sqrt{T\log (dT)}$) with (resp. without) the margin condition. TH Lasso bandit removes the $\log d$ and $\log T$ multiplicative factors. In most applications of the sparse linear contextual bandit, both $T$ and $d$ are typically very large, and the regret improvement obtained by TH Lasso bandit is significant. 
Also note that our regret upper bounds match the minimax lower bound $\Omega(\sqrt{s_0 T}) $ proved in \citet{ren2020dynamic}.




\subsection{Sketch of the Proof of Theorems}

We sketch below the proof of Theorem \ref{thm:regret_ub_klarge} and \ref{thm:regret_ub_wo_margin_klarge}. Complete proofs of Theorems and associated Lemmas are presented in Appendix~\ref{sec:Proof_theorems} and Appendix~\ref{sec:proof_lemmas_klarge}, respectively.

\paragraph{(1) Estimation of the Support of $\theta$.} First, we prove that the estimated support contains the true support $S(\theta)$ with high probability.

\begin{lemma}\label{lm:support_recovery_klarge}
 Let $t \ge  \frac{2 \log (2 d^2)}{C_0^2}$ such that $4 \left( \frac{4 \nu C_{\textnormal{b}} s_0}{\phi_0^2} + \sqrt{\left(1 + \frac{4\nu C_{\textnormal{b}}}{\phi_0^2}\right)s_0}\right)\lambda_t \le \theta_{\min}$. Under Assumptions \ref{asm:sparsity_param_klarge}, \ref{asm:comp_cond}, \ref{asm:relax_sym}, and \ref{asm:balanced_cov}, 
$
    \Pr \left(S(\theta) \subset \hat{S}_1^{(t)} \text{ and } |\hat{S}_1^{(t)} \setminus S(\theta)| \le \frac{4\nu C_{\textnormal{b}} \sqrt{s_0}}{\phi^2_0}\right)
    $
    $
     \ge 1 -  2 \exp\left( -\frac{t \lambda_t^2}{32 \sigma^2 s_A^2} + \log d\right) - \exp\left( - \frac{t C_0^2}{2}\right).
$
\end{lemma}
\noindent Lemma~\ref{lm:support_recovery_klarge} extends the support recovery result of the Thresholded Lasso \cite{zhou2010thresholded} to the case of non-i.i.d data (generated by the bandit algorithm). 
The dependence on $s_0$ is analogous to the offline result (Theorem~3.1 of \citet{zhou2010thresholded}). As it can be seen from the proof, even after the single-step thresholding, for all sufficiently large $t$, we have the guarantee of $S(\theta) \subset \hat{S}_0^{(t)}$ and $ | \hat{S}_0^{(t)} \setminus S(\theta)| = \mathcal{O}(s_0)$ with high probability. However, with the two-step thresholding, we have $ | \hat{S}_1^{(t)} \setminus S(\theta)| = \mathcal{O}(\sqrt{s_0})$ (See Appendix~\ref{app:benefit_thresholding} for the benefit of the two-step thresholding in detail). 

\begin{remark}
In the proof of Lemma~\ref{lm:support_recovery_klarge}, we also obtain an bound on the estimation error of $\hat{\theta}_0^{(t)}$ (by the Lasso).
One may directly use $\hat{\theta}_0^{(t)}$ for the arm selection as is in \citet{oh2020sparsity}, however, this results in a weaker performance guarantee of the order $\mathcal{O} ( \log d + \sqrt{T \log (dT)})$ (without the margin condition).
This is due to the fact that the estimation error of $\hat{\theta}_0^{(t)}$ has a dependence on $d$, which impacts the order of the regret. 
This motivates the use of the thresholding procedure. With this procedure (i.e., using $\hat{\theta}_t$), we remove the dependence in $d$ of the estimation error when $t$ is larger than $\tau$, which, in turn, leads to an instantaneous regret bound independent of $d$. In summary, the thresholding procedure allows us to derive better regret bounds than those in existing work (e.g., \citet{oh2020sparsity}).
\end{remark}

Define
    $\mathcal{E}_t \coloneqq \left\{S(\theta) \subset \hat{S}_1^{(t)} \;\text{and}\; |\hat{S}_{1}^{(t)} \setminus S(\theta)| \le  \frac{4 \nu C_{\textnormal{b}} \sqrt{s_0}}{\phi^2_0} \right\}.$
In the remaining of the proof, in view of Lemma~\ref{lm:support_recovery_klarge}, we can assume that the event $\mathcal{E}_t$ holds.

\paragraph{(2) Minimal Eigenvalue of the Empirical Gram Matrix.}  
We write $\hat{S}_1^{(t)} = \hat{S}$ for the simplicity. Let $\hat{\Sigma}_{\hat{S}} \coloneqq \frac{1}{t} \sum_{s = 1}^t A_{s}(\hat{S})  A_{s}(\hat{S})^\top$ be the empirical Gram matrix on the estimated support.  We prove that the positive definiteness of the empirical Gram matrix on the estimated support is guaranteed. 
\begin{lemma}\label{lm:lowerbound_eig_S_klarge}
 Let $t \in [T]$. Under Assumptions \ref{asm:sparsity_param_klarge} and \ref{asm:cov_div_klarge}, we have:
$
    \Pr\left(\lambda_{\min} (\hat{\Sigma}_{\hat{S}}) \ge   \frac{\alpha}{4\nu  C_{\textnormal{b}}} \ \big| \ \mathcal{E}_t \right)   \ge 1 -  \exp\left( \log\left(s_0 + \frac{4 \nu C_{\textnormal{b}}\sqrt{s_0}}{\phi_0^2} \right)
 - \frac{t \alpha}{20 s_A^2\nu C_{\textnormal{b}}\left(s_0 + (4 \nu C_{\textnormal{b}} \sqrt{s_0})/\phi_0^2\right) } \right). 
$
\end{lemma}

\paragraph{(3) Estimation of $\theta$ after Thresholding.} Next, we study the accuracy of $\hat{\theta}_{t}$.

\begin{lemma}\label{lm:LS_estim_risk_klarge}
 Let $t \in [T]$ and $s' = s_0 + 4 \nu C_{\textnormal{b}} \sqrt{s_0}/\phi_0^2$. Under Assumption~\ref{asm:sparsity_param_klarge}, we have, for all $x, \lambda >0$:
$
     \Pr \left( \|\hat{\theta}_{t+1} - \theta \|_2 \ge x \; \text{and} \;\lambda_{\min}(\hat{\Sigma}_{\hat{S}}) \ge \lambda \ \big| \ \mathcal{E}_t \right)  
$
$
\le2 s' \exp \left( - \frac{\lambda^2 t x^2}{2 \sigma^2 s_A^2 s'}\right).$
\end{lemma}

From the above lemma, we conclude that $\theta$ is well estimated with high probability. Note that in the above estimation error, the dependency in $s_0$ can be also improved from linear to square root compared with the analysis of Lemma~1 (Oracle inequality) in \citet{oh2020sparsity} (SA Lasso bandit). This stems from the fact that using the compatibility condition, one can only control the $\ell_1$ norm of the estimation error of $\theta$, while using the OLS leads to an $\ell_2$ guarantee. 

\paragraph{(4) Instantaneous Regret Upper Bound with the Margin Condition.}
For the previous lemmas, we can derive an upper bound on the instantaneous regret with the margin condition. Define $h_0 = \lfloor \sqrt{\log(4 (s_0 + \frac{4 \nu C_{\textnormal{b}}\sqrt{s_0}}{\phi_0^2}))}  + 1 \rfloor$.
 
\begin{lemma}[With the margin condition]\label{lm:inst_regret_bound_klarge}
Define $\mathcal{G}_{t}^{\frac{\alpha}{4\nu C_{\textnormal{b}}}} \coloneqq \left\{\lambda_{\min } ( \hat{\Sigma}_{\hat{S}} ) \ge \frac{\alpha}{4\nu C_{\textnormal{b}}} \right\}$. Let $t \ge 2$. Under Assumptions \ref{asm:sparsity_param_klarge}, \ref{asm:comp_cond}, \ref{asm:relax_sym}, \ref{asm:balanced_cov}, \ref{asm:cov_div_klarge}, and \ref{asm:margin}, the expected instantaneous regret $\EXP[\max_{A \in \mathcal{A}_t} \langle A - A_t, \theta \rangle]$ is upper bounded by:
\begin{align*}
& \frac{1408 \sigma^2 s_A^4 C_{\textnormal{m}} (K-1) h_0^3 \nu^2 C_{\textnormal{b}}^2 \left(s_0 + \frac{4 \nu C_{\textnormal{b}}\sqrt{s_0}}{\phi_0^2}\right)}{\alpha^2} \frac{1}{t - 1} 
\\
& + 2 (K-1)  s_A s_1  \left(\Pr(\mathcal{E}_t^c) + \Pr\left(\left(\mathcal{G}_{t}^{\frac{\alpha}{4 \nu C_{\textnormal{b}}}}\right)^c \middle| \mathcal{E}_t\right) \right).
\end{align*}
\end{lemma}
Notice that the first term of this instantaneous regret bound does not depend on $d$. This leads to the better regret order.

On the other hand, without the margin condition, we present the key lemma, which is proven by a novel application of the discretization technique:
\begin{lemma}[Without the margin condition]\label{lm:inst_regret_bound_wo_margin_klarge}
Under Assumptions \ref{asm:sparsity_param_klarge},  \ref{asm:comp_cond},  \ref{asm:relax_sym}, \ref{asm:balanced_cov}, and \ref{asm:cov_div_klarge}, for any $t \in [T]$, $\EXP[\max_{A \in \mathcal{A}_t} \langle A - A_t, \theta\rangle]$ is upper bounded by
\begin{align*}
& \frac{36 \sigma s_A  (K-1) h_0^2 \nu C_{\textnormal{b}}}{\alpha}\sqrt{\frac{2 \left(s_0 + \frac{4 \nu C_{\textnormal{b}}\sqrt{s_0} }{\phi_0^2}\right)}{t-1}}
\\
& + 2  (K-1) s_A s_1  \left(\Pr(\mathcal{E}_t^c) + \Pr\left(\left(\mathcal{G}_{t}^{\frac{\alpha}{4\nu C_{\textnormal{b}}}}\right)^c \middle| \mathcal{E}_t\right) \right).
\end{align*}
\end{lemma}
Again, the first term in the above bound is independent of $d$. Note also that compared to existing work, we improve the dependence in $t$: we get $1/\sqrt{t}$ instantaneous upper bound while in the other recent work (e.g., \citet{kim2019doubly, oh2020sparsity}) they get $\sqrt{\log t /t}$. As a consequence, we obtain better regret guarantees without the margin condition. More precisely, we manage to remove the unnecessary $\log T$ factors in the regret that was present in all previous studies.


By summing up these instantaneous regret bounds, we get Theorem~\ref{thm:regret_ub_klarge} and \ref{thm:regret_ub_wo_margin_klarge}. 
In Appendix~\ref{sec:additional_theorems}, we also provide regret guarantees without Assumption~\ref{asm:balanced_cov} but when $K=2$ (Theorem~\ref{thm:regret_ub_k2}) and without the margin condition (Theorem~\ref{thm:regret_ub_wo_margin_k2}). 
These theorems are established using the relaxed symmetry assumption only; see also the proof of Lemma~2 in \citet{oh2020sparsity}.


\input{experiment}

\section{Conclusion}
In this paper, we studied the high-dimensional contextual linear bandit problem with sparsity. We devised TH Lasso bandit, a simple algorithm that applies a Lasso procedure with thresholding  to estimate the support of the unknown parameter. We established finite-time regret upper bounds under various assumptions, and in particular with and without the margin condition. These bounds exhibit a better regret scaling than those derived for previous algorithms. We also numerically compared TH Lasso bandit to previous algorithms in a variety of settings, and showed that it outperformed other algorithms in these settings. 


In future work, it would be interesting to consider scenarios where the assumptions made in this paper may not hold. In particular, it is worth investigating the case where the relaxed symmetry condition (Assumption~\ref{asm:relax_sym}) is not satisfied. In this case, being greedy in the successive arm selections may not work. It is intriguing to know whether devising an algorithm without forced uniform exploration and with reasonable regret guarantees is possible. 


\section*{Acknowledgements}

We would like to thank Komei Fujita, Yusuke Kaneko, Hiroaki Shiino, and Shota Yasui for the fruitful discussions. 
We also thank anonymous reviewers for helpful comments on the previous version of our manuscript.
K. Ariu was partially supported by the Nakajima Foundation Scholarship. A. Proutiere's research is partially supported by the Wallenberg AI, Autonomous Systems and Software Program (WASP) funded by the Knut and Alice Wallenberg Foundation, and by Digital Futures.

==> Lasso Bandits_arXiv/defs.tex <==

\usepackage[utf8]{inputenc} %
\usepackage[T1]{fontenc}    %
\usepackage{titletoc}
\usepackage{hyperref}       %
\usepackage{url}            %
\usepackage{booktabs}       %
\usepackage{amsfonts}       %
\usepackage{nicefrac}       %
\usepackage{microtype}      %
\usepackage{xcolor}         %




  
\newcommand{\argmax}{\mathop{\rm argmax}\limits}
\newcommand{\argmin}{\mathop{\rm argmin}\limits}

\newcommand{\ep}{\hfill $\Box$}


\usepackage{bbm}
\usepackage{paralist}
\usepackage{enumitem}
\usepackage{xcolor}
\usepackage{mathtools}
\usepackage{url}


\usepackage{dsfont}



\renewcommand{\vec}{\boldsymbol}
\DeclareMathOperator{\KL}{\textnormal{kl}}

\DeclareMathOperator{\EXP}{\mathbb{E}}
\newcommand{\qand}{\quad \text{and} \quad}

\renewcommand{\tilde}{\widetilde}

\renewcommand{\Pr}{\mathbb{P}}
\renewcommand{\star}{*}
\newcommand{\iid}{\textnormal{iid}}
\newcommand{\alg}{\textnormal{DEL}}
\newcommand{\kl}{\textnormal{kl}}
\newcommand{\tv}{\textnormal{TV}}
\newcommand{\note}[1]{{\color{blue} \tt #1}}
\newcommand{\TN}{\textnormal}


\newcommand{\est}{\textnormal{est}}
\newcommand{\mnt}{\textnormal{mnt}}
\newcommand{\xpt}{\textnormal{xpt}}
\newcommand{\xpr}{\textnormal{xpr}}
\newcommand{\indicator}{\mathds{1}}

\usepackage{pdfrender}
\newcommand*{\boldcheckmark}{%
  \textpdfrender{
    TextRenderingMode=FillStroke,
    LineWidth=.5pt, %
  }{\checkmark}%
}

\renewcommand{\cite}{\citep}




\usepackage{tablefootnote}

==> Lasso Bandits_arXiv/experiment.tex <==
\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=1.1\textwidth]{figs/synthetic/experiment1/K2_d1000_s5_xm10_rho0.7_theta1/regrets_scale_main.pdf}
    \end{minipage}
    \begin{minipage}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=1.1\textwidth]{figs/synthetic/experiment1/K2_d2000_s20_xm10_rho0.7_theta1/regrets_scale_main.pdf}
    \end{minipage}
    \begin{minipage}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=1.1\textwidth]{figs/synthetic/experiment1/K2_d10000_s20_xm10_rho0.7_theta1/regrets_scale_main.pdf}
    \end{minipage} \\
    \begin{minipage}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=1.1\textwidth]{figs/synthetic/experiment1/K50_d1000_s5_xm10_rho0.7_theta1/regrets_scale_main.pdf}
    \end{minipage}
    \begin{minipage}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=1.1\textwidth]{figs/synthetic/experiment1/K50_d2000_s20_xm10_rho0.7_theta1/regrets_scale_main.pdf}
    \end{minipage}
    \begin{minipage}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=1.1\textwidth]{figs/synthetic/experiment1/K50_d10000_s20_xm10_rho0.7_theta1/regrets_scale_main.pdf}
    \end{minipage}
    \caption{Cumulative regret of the three algorithms with $\rho^2=0.7$, $A_{\max}=10$ in six scenarios selected using $K\in \{2, 50\}$, $d\in \{1000, 2000, 10000\}$, and $s_0\in \{5, 20\}$.
    The shaded area represents the standard errors.}
    \label{fig:experiment1_regrets}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \begin{minipage}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=1.1\textwidth]{figs/synthetic/experiment1/K2_d1000_s5_xm10_rho0.7_theta1/false_positive.pdf}
    \end{minipage}
    \begin{minipage}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=1.1\textwidth]{figs/synthetic/experiment1/K2_d1000_s5_xm10_rho0.7_theta1/false_negative.pdf}
    \end{minipage}
    \begin{minipage}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=1.1\textwidth]{figs/synthetic/experiment1/K2_d1000_s5_xm10_rho0.7_theta1/error_l2.pdf}
    \end{minipage}
    \caption{(Left) Number of false positives $|\hat{S}_1^{(t)} \setminus S(\theta)|$, (center) false negatives $|S(\theta) \setminus \hat{S}_1^{(t)}|$, (right) $\ell_2$-norm error $\|\hat{\theta}_t - \theta\|_2$ of the three algorithms with $\rho^2=0.7$, $A_{\max}=10$, $K=2$, $s_0=5$, and $d=1000$. The shaded area represents the standard errors.}
    \label{fig:experiment1_error}
\end{figure*}

\begin{figure*}[t!]
\begin{minipage}{0.48\textwidth}
\centering
\includegraphics[width=0.96\textwidth]{figs/synthetic/experiment2/K2_d1000_s5_regrets.pdf}
\caption{Cumulative regret at round $t=1000$ of TH Lasso bandit and SA Lasso bandit with $\rho^2=0.7$, $K=2$, $d=1000$, $s_0=5$, and varying $A_{\max}\in \{2.5, 5, 10, 20, 40, \infty\}$.
The error bars represent the standard errors.}
\label{fig:experiment2_regrets}
\end{minipage}
\hfill
\begin{minipage}{0.48\textwidth}
\centering
\includegraphics[width=0.96\textwidth]{figs/synthetic/discussion/regrets.pdf}
\caption{Cumulative regret at round $t=1000$ of TH Lasso bandit and SA Lasso bandit with $\rho^2=0.7$, $A_{\max}=10$, $K=2$, $d=1000$, $s_0=5$, and varying $\lambda_0/\lambda^{\ast}\in [0.1, 2.5]$.
The error bars represent the standard errors.}
\label{fig:discussion_regrets}
\end{minipage}
\end{figure*}

\section{Experiments}

In this section, we empirically evaluate the TH Lasso bandit algorithm. 
We compare its performance to those of the Lasso Bandit \cite{bastani2020online}, Doubly-Robust (DR) Lasso bandit \cite{kim2019doubly}, and SA Lasso bandit \cite{oh2020sparsity} algorithms. Note that the Lasso bandit algorithm \cite{bastani2020online} deals with a slightly different problem setting ($\theta$ varies across arms in their setting). We follow the comparison ideas in \citet{kim2019doubly} (considered the $Kd$-dimensional context vectors and the $Kd$-dimensional regression parameters for each arm. For details, see \citet{kim2019doubly}).

\paragraph{Reward Parameter and Contexts.} We consider problems where $\theta\in \mathbb{R}^d$ is sparse, i.e., $\|\theta\|_0=s_0$. We generate each non-zero components of $\theta$ in an i.i.d. manner using the uniform distribution on $[1, 2]$.
In each round $t$, for each component $i\in [d]$, we sample $((A_{t,1})_{i}, \cdots, (A_{t,K})_{i})^{\top} \in \mathbb{R}^K$ from a Gaussian distribution $\mathcal{N}(\mathbf{0}_{K}, V)$ where $V_{i,i}=1$ for all $i\in [K]$ and $V_{i,k}=\rho^2=0.7$ for all $i\neq k\in [K]$. We then normalize each $A_{t,k} = ((A_{t,k})_1, \ldots, (A_{t,k})_d)^{\top} \in \mathbb{R}^d$ so that its $\ell_2$-norm is at most $A_{\max}$ for all $k \in [K]$.
Note that the components of the feature vectors are correlated over $[d]$ and over $[K]$. The noise process is Gaussian, i.i.d. over rounds: $\varepsilon_t\sim\mathcal{N}(0, 1)$. We test the algorithms for different values of $K, d, s_0$, and $A_{\max}$. For each experimental setting, we averaged the results for $20$ instances. We also provide additional experimental results with non-Gaussian distributions in Appendix~\ref{sec:exp_non_gaussian}.

\begin{remark}
In most of our experiments, the context is drawn from a multivariate Gaussian, or uniform distribution on $[-1,1]^d$.
In this case, the minimum eigenvalue of the gram matrix $\Sigma$ is lower bounded by some constant. 
Hence, Assumptions~\ref{asm:comp_cond} and \ref{asm:cov_div_klarge} are satisfied. 
Clearly, Assumption~\ref{asm:relax_sym} is satisfied by the symmetry of the distribution. 
When the distribution is independent over the arms, from Proposition~1 in \citet{oh2020sparsity}, Assumption~\ref{asm:balanced_cov} is satisfied. 
Since each element of the context distribution has a bounded density everywhere, Assumption~\ref{asm:margin} is also satisfied. 
Furthermore, in Appendix~\ref{subsec:numerical_hard_instances}, we empirically tested our algorithm for some hard problems where the covariate diversity condition \cite{bastani2021mostly} does not hold. 
\end{remark}


\paragraph{Algorithms.} For DR Lasso bandit and Lasso bandit, we use the tuned hyperparameter at\\ \url{https://github.com/gisoo1989/Doubly-Robust-Lasso-Bandit}.\\
For the SA Lasso bandit and TH Lasso bandit algorithms, we tune the hyperparameter $\lambda_0$ in $[0.01, 0.5]$ to roughly optimize the algorithm performance when $K=2, d=1000, A_{\max}=10$, and $s_0=5$. As a result, we set $\lambda_0=0.16$ for SA Lasso bandit, and set $\lambda_0=0.02$ for TH Lasso bandit.


\paragraph{Results.} We first compare the regret of each algorithm with $A_{\max}=10$, $K\in\{2, 50\}$, $d=\{1000, 2000, 10000\}$, and $s_0\in \{5, 20\}$. We experimented with larger values of $d$, in addition to the one in existing studies.
Figure~\ref{fig:experiment1_regrets} shows the average cumulative regret for each algorithm.
We find that TH Lasso bandit outperforms the other algorithms in all scenarios. We provide additional experimental results, including experiments with different correlation levels $\rho^2(\in\{0, 0.3\})$ and dimension $d$, in Appendix~\ref{sec:exp_non_gaussian}. 

Next, we compare the estimation accuracy for $\theta$ under  three algorithms (DR, SA, and TH Lasso bandit) in the scenario: $K=2, d=1000, A_{\max}=10, s_0=5$.
Figure~\ref{fig:experiment1_error} shows the number of false positives $|\hat{S}_1^{(t)} \setminus S(\theta)|$, the number of false negatives $|S(\theta) \setminus \hat{S}_1^{(t)}|$, and $\ell_2$-norm error $\|\hat{\theta}_t - \theta\|_2$.
Note that, for DR Lasso bandit and SA Lasso bandit, we define the estimated support as $\hat{S}_1^{(t)}=\{i\in [d]: \hat{\theta}_{t,i}\neq 0\}$. We can observe that the number of false positives of our algorithm converge to zero faster than those of DR Lasso bandit and SA Lasso bandit.
Furthermore, our algorithm yields a smaller estimation error $\|\hat{\theta}_t - \theta\|_2$ than the two other algorithms, as is shown in right column of Figure~\ref{fig:experiment1_error}.

We also conduct experiments varying $A_{\max}\in \{2.5, 5, 10, 20, 40, \infty\}$. As in the previous experiments, for each $A_{\max}$, we normalize each feature vector $A_{t,k}$ so that its $\ell_2$-norm is at most $A_{\max}$ for all $k \in [K]$.
We set $K=2, d=1000$, and $s_0=5$. Figure~\ref{fig:experiment2_regrets} shows the average cumulative regret at $t=1000$ of TH Lasso bandit and SA Lasso bandit for each $A_{\max}$. This experiment confirms that TH Lasso exhibits lower regret than SA Lasso bandit. Additional results when $K=50$ and $s_0=20$ are also included in Appendix~\ref{subsec:additional_Amax}.

Finally, we examine the robustness of TH Lasso bandit and SA Lasso bandit with respect to the hyperparameter $\lambda_0$. We vary $\lambda_0 \in [0.1\lambda^{\ast}, 2.5\lambda^{\ast}]$ where $\lambda^{\ast}= 0.02$ for TH Lasso bandit and $\lambda^{\ast}= 0.16$ for SA Lasso bandit. We set $K=2, d=1000, s_0=5$, and $A_{\max}=10$. Figure~\ref{fig:discussion_regrets} shows the average cumulative regret at $t=1000$ for TH Lasso bandit and SA Lasso bandit for different ratios $\lambda_0/\lambda^{\ast}$.
Observe that the regret of TH Lasso bandit is more stable than that of SA Lasso bandit as the  ratio grows. Indeed, the performance of TH Lasso bandit is not very sensitive to the choice of $\lambda_0$: it is robust. This contrasts with the SA Lasso bandit algorithm, for which a careful tuning of $\lambda_0$ is needed to get good performance.



==> Lasso Bandits_arXiv/latexmkrc <==
$latex = 'platex';
$bibtex = 'pbibtex';
$dvipdf = 'dvipdfmx %O -o %D %S';
$makeindex = 'mendex %O -o %D %S';
$pdf_mode = 3; 

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

==> latexmkrc <==
$latex = 'platex';
$bibtex = 'pbibtex';
$dvipdf = 'dvipdfmx %O -o %D %S';
$makeindex = 'mendex %O -o %D %S';
$pdf_mode = 3; 

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
